IL-TUR: Benchmark for Indian Legal Text Understanding and Reasoning

Legal systems worldwide are inundated with exponential growth in cases and documents. There is an imminent need to develop NLP and ML techniques for automatically processing and understanding legal documents to streamline the legal system. However, evaluating and comparing various NLP models designed specifically for the legal domain is challenging. This paper addresses this challenge by proposing IL-TUR: Benchmark for Indian Legal Text Understanding and Reasoning. IL-TUR contains monolingual (English, Hindi) and multi-lingual (9 Indian languages) domain-specific tasks that address different aspects of the legal system from the point of view of understanding and reasoning over Indian legal documents. We present baseline models (including LLM-based) for each task, outlining the gap between models and the ground truth. To foster further research in the legal domain, we create a leaderboard (available at: https://exploration-lab.github.io/IL-TUR/) where the research community can upload and compare legal text understanding systems.

==> sections/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please read the checklist guidelines carefully for information on how to answer these questions.  For each question, change the default \answerTODO{} to \answerYes{},\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf justification to your answer}, either by referencing the appropriate section of your paper or providing a brief inline description.  For example:

% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

%\answerTODO{}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \textcolor{blue}{\textbf{Yes}}
  \item Did you describe the limitations of your work?
   \textcolor{blue}{\textbf{Yes in Appendix \ref{sec:limitations}}}
  \item Did you discuss any potential negative societal impacts of your work?
    \textcolor{blue}{\textbf{NA}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \textcolor{blue}{\textbf{Yes in Appendix \ref{sec:ethics}}}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
     \textcolor{blue}{\textbf{NA}}
	\item Did you include complete proofs of all theoretical results?
    \textcolor{blue}{\textbf{NA}}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \textcolor{blue}{\textbf{Yes, in the Github Repo and Appendix}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \textcolor{blue}{\textbf{Yes, in the Github Repo and Appendix}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \textcolor{blue}{\textbf{Yes, in the Github Repo and Appendix}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \textcolor{blue}{\textbf{Yes, in the Github Repo and Appendix}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \textcolor{blue}{\textbf{Yes, Section 3 and 4}}
  \item Did you mention the license of the assets?
    \textcolor{blue}{\textbf{Yes, Section 3 and 4}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \textcolor{blue}{\textbf{Yes, Github Repo and Appendix}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \textcolor{blue}{\textbf{NA}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
   \textcolor{blue}{\textbf{Yes, Section 3, 4 and Appendix}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \textcolor{blue}{\textbf{NA}}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \textcolor{blue}{\textbf{NA}}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \textcolor{blue}{\textbf{NA}}
\end{enumerate}

\end{enumerate}
